Spin orbit-induced anisotropic conductivity of a disordered 2DEG

We present a semi-automated computer-assisted method to generate and calculate diagrams in the disorder averaging approach to disordered 2D conductors with intrinsic spin-orbit interaction (SOI). As an application, we calculate the effect of the SOI on the charge conductivity for disordered 2D systems and rings in the presence of Rashba and Dresselhaus SOI. In an infinite-size 2D system, anisotropic corrections to the conductivity tensor arise due to phase-coherence and the interplay of Rashba and Dresselhaus SOI. The effect is more pronounced in the quasi-onedimensional case, where the conductivity becomes anisotropic already in the presence of only one type of SOI. The anisotropy further increases if the time-reversal symmetry of the Hamiltonian is broken.

==> 6.ins.tex <==
\begin{picture}(0,0)%
\includegraphics{6}%
\end{picture}%
\setlength{\unitlength}{4144sp}%
%
\begingroup\makeatletter\ifx\SetFigFontNFSS\undefined%
\gdef\SetFigFontNFSS#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(8867,4197)(2917,-4703)
\end{picture}%


==> _region_.tex <==
\message{ !name(zla.tex)}%-*-EMaxima-*-
% см. ~/PA6OTA/MAXIMA/emaxima.tex
\input{header-landscape.tex}
\addtolength{\oddsidemargin}{.2cm}
\usepackage{emaxima}
% Чтобы следующие команды сработали, следует везде заменить:  \$ --> \var и убрать \mathrm
\newcommand{\varnt}{\tilde n} \newcommand{\varx}{x} \newcommand{\varxa}{x_a} \newcommand{\varxb}{x_b} \newcommand{\varm}{m} \newcommand{\vardel}{\delta}
\newcommand{\varDel}{\Delta} \newcommand{\varEFt}{\EF\tau}
% А ещё надо бы перейти от \pmatrix к \begin{pmatrix}...\end{pmatrix}
\begin{document}

\message{ !name(zla.tex) !offset(-3) }

\begin{maxima}
kill(mp,plusTOlist,xx,map2,fun,massiv,xi,pf,x,xa,xb,tau,Del,grinv,gainv,grp,grm,gap,gam,nt,m,EF,xiEF,EFt)$ declare([xi,t,ntildy],real)$
assume(tau>0,ntildy>0,m>0,EFt>0)$
plusTOlist(xx):=if atom(xx) then [xx] elseif op(xx)="+" then args(xx) elseif op(xx)="[" then xx else [xx]$
map2(fun,massiv):=map(lambda([xx],  map(fun, xx)), massiv)$
grinv:-xi+%i/(2*tau)$ gainv:conjugate(grinv)$ gr:1/grinv$ ga:1/gainv$
grp:1/(grinv+Del/2); grm:1/(grinv-Del/2)$ gap:1/(gainv+Del/2)$ gam:1/(gainv-Del/2)$
ntExpr:sqrt((1+del)*cos(phi)^2+(1-del)*sin(phi)^2);
\maximaoutput*
\m  {{1}\over{-\xi+{{i}\over{2\,\tau}}+{{\mathrm{\$Del}}\over{2}}}} \\
\m  \sqrt{\left(\cos \varphi\right)^2\,\left(\mathrm{\%del}+1\right)+\left(\sin \varphi\right)^2\,\left(1-\mathrm{\%del}\right)} \\
\end{maxima}
\begin{maxima}
res1:matrixmap(lambda([yy],block([resA,resB,resC],
resA:subst([xi=z/tau,EF=EFt/tau],subst([p=sqrt(2*m*(EF+EF*xiEF)),pf=sqrt(2*m*EF)],subst([px=p*cos(phi),py=p*sin(phi),Del=2*p*nt*x/(2*pf*tau)],yy))),
resB:map(factor,plusTOlist(subst([xiEF=z/EFt],ratdisrep(taylor(resA,xiEF,0,2))))),
resC:map(lambda([xx],factor(1/tau*integrate(xx,z,-inf,inf))),resB),
expand(1/(2*%pi)*integrate(subst([nt=ntExpr],apply("+",resC)),phi,0,2*%pi)))),
m/(2*%pi)*diag_matrix(px^2,py^2)/m^2*(grp*gap+grm*gam-2*gr*ga));
\maximaoutput*
\m  \begin{pmatrix}{{{\mathrm{\$x}^2\,\mathrm{\%del}}\over{4\,\mathrm{\$EFt}}}+{{\mathrm{\$x}^2}\over{2\,\mathrm{\$EFt}}}&0\cr 0&{{\mathrm{\$x}^2}\over{2\,\mathrm{\$EFt}}}-{{\mathrm{\$x}^2\,\mathrm{\%del}}\over{4\,\mathrm{\$EFt}}}\cr }\end{pmatrix} \\
\end{maxima}
\begin{maxima}
h[i,j]:=[(xa+xb)^2,(xa-xb)^2][i]/(2*pf*tau)^2*2*[px,py][i]*[px,py][j]/(Del*m)$
res2:matrixmap(lambda([yy],block([resA,resB,resC],
resA:subst([xi=z/tau,EF=EFt/tau],subst([p=sqrt(2*m*(EF+EF*xiEF)),pf=sqrt(2*m*EF)],subst([px=p*cos(phi),py=p*sin(phi),Del=2*p*nt*x/(2*pf*tau)],yy))),
resB:map(factor,plusTOlist(subst([xiEF=z/EFt],ratdisrep(taylor(resA,xiEF,0,2))))),
resC:map(lambda([xx],factor(1/tau*integrate(xx,z,-inf,inf))),resB),
expand(1/(2*%pi)*integrate(subst([nt=ntExpr],apply("+",resC)),phi,0,2*%pi)))),
m/(2*%pi)*genmatrix(h,2,2)*(grm*gam-grp*gap));
\maximaoutput*
\m  \begin{pmatrix}{-{{\mathrm{\$xb}^2}\over{4\,\mathrm{\$EFt}}}-{{\mathrm{\$xa}\,\mathrm{\$xb}}\over{2\,\mathrm{\$EFt}}}-{{\mathrm{\$xa}^2}\over{4\,\mathrm{\$EFt}}}&0\cr 0&-{{\mathrm{\$xb}^2}\over{4\,\mathrm{\$EFt}}}+{{\mathrm{\$xa}\,\mathrm{\$xb}}\over{2\,\mathrm{\$EFt}}}-{{\mathrm{\$xa}^2}\over{4\,\mathrm{\$EFt}}}\cr }\end{pmatrix} \\
\end{maxima}
\begin{maxima}
fiRes:subst([del=2*xa*xb/x^2],res1+res2);
fiRes[1,1]-fiRes[2,2];
\maximaoutput*
\m  \begin{pmatrix}{-{{\mathrm{\$xb}^2}\over{4\,\mathrm{\$EFt}}}-{{\mathrm{\$xa}^2}\over{4\,\mathrm{\$EFt}}}+{{\mathrm{\$x}^2}\over{2\,\mathrm{\$EFt}}}&0\cr 0&-{{\mathrm{\$xb}^2}\over{4\,\mathrm{\$EFt}}}-{{\mathrm{\$xa}^2}\over{4\,\mathrm{\$EFt}}}+{{\mathrm{\$x}^2}\over{2\,\mathrm{\$EFt}}}\cr }\end{pmatrix} \\
\m  0 \\
\end{maxima}
\end{document}

\message{ !name(zla.tex) !offset(-56) }


==> cond.ins.tex <==
\begin{picture}(0,0)%
\includegraphics{cond}%
\end{picture}%


==> other.tex <==
\section{Universal and non-universal contributions\label{sec:uniIneuni}}
%\msc{This section is still unsatisfactory, to be updated\ldots}
In the diagrammatic technique, one often has to take integrals from the product of GFs of the type
\begin{equation}\label{algProGF}
\ipd\prod_{i=1}^n\GR(\vec p-{\vec q}_i)\prod_{j=1}^m\GA(\vec p-{\vec q}_j).
\end{equation}
In case when all momenta arguments are equal in~\eqref{algProGF}, $\forall i,j$ ${\vec q}_i={\vec q}_j=0$, the integral is taken using the change of
variable: $\ipds\to\nu\int_{-\EF}^{\infty}\ud\xi$, where the density of states $\nu=m/(2\pi\hbar)$ in 2D.
About such integrals, we will say that ``integral $J=\int_{-\EF}^{\infty}f(\xi)\ud\xi$ converges on the scale $\delta\xi$'', if
$J_{\delta\xi}\equiv\int_{-\delta\xi}^{\delta\xi}f(\xi)\ud\xi$ has the same order of magnitude (in $\pf l\gg\hbar$) as $J$.

An integral $\int\ud\xi$ from the product of GFs is of the order of $m\tau^{h-1}$ if  it  converges on the scale $\delta\xi\sim\hbar/\tau$:
\begin{equation}\label{epGF}
\int\ud\xi\GR^n(\xi)\GA^m(\xi)\sim\tau^{n+m-1}.
\end{equation}
The simplest example of \eqref{epGF} is a ``bubble'' $\nu\int\ud\xi\GR(\xi)\GA(\xi)=2\pi\nu\tau$. It is \emph{universal}, because only values of
$\xi=\epsilon_{\vec p}-\EF$ out of close vicinity of zero (i.e., $\epsilon_{\vec p}\in[\EF-\hbar/\tau,\EF+\hbar/\tau]$) contribute to the result. Only in this close
vicinity of the Fermi level Landau Fermi liquid theory is valid.

Other integrals, e.g., $\int\ud\xi\GR^2(\xi)$, we call \emph{non-universal}. Using~\eqref{agf}, one concludes that
\begin{equation}\label{estNU}
\ipd\GR^2(\vec p)\sim\frac\hbar{\EF\tau}\ipd\GR(\vec p)\GA(\vec p).
\end{equation}
\ldots
\msc{Still we have to say smth about the non-universal corrections\ldots}

In conclusion, the universal corrections are produced by $\int\ud\xi\GR^n\GA^m$;
all other contributions must be neglected by postulating $\ipds\equiv\nu\int_{-\infty}^\infty\ud\xi$.

The above reasoning is valid also in case when the momentum arguments in~\eqref{algProGF} are close to each other (the s.c. diffusion approximation):
\begin{equation}
\forall i\quad q_il\ll\hbar.
\end{equation}
We call momentum variables ${\vec q}_i$ ``small'' if $q_il\ll\hbar$. Then $q_i\ll p\sim\pf$; we call $\vec p$ ``large'' momentum variable.


==> rv1.ins.tex <==
\begin{picture}(0,0)%
\includegraphics{rv1}%
\end{picture}%
\setlength{\unitlength}{3947sp}%
%
\begingroup\makeatletter\ifx\SetFigFontNFSS\undefined%
\gdef\SetFigFontNFSS#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(494,944)(269,-681)
\end{picture}%


==> rv2.ins.tex <==
\begin{picture}(0,0)%
\includegraphics{rv2}%
\end{picture}%
\setlength{\unitlength}{3947sp}%
%
\begingroup\makeatletter\ifx\SetFigFontNFSS\undefined%
\gdef\SetFigFontNFSS#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(494,944)(269,-681)
\end{picture}%


==> rv3.ins.tex <==
\begin{picture}(0,0)%
\includegraphics{rv3}%
\end{picture}%
\setlength{\unitlength}{3947sp}%
%
\begingroup\makeatletter\ifx\SetFigFontNFSS\undefined%
\gdef\SetFigFontNFSS#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(2503,1052)(1252,-734)
\end{picture}%


==> wl0.ins.tex <==
\begin{picture}(0,0)%
\includegraphics{wl0}%
\end{picture}%
\setlength{\unitlength}{3947sp}%
%
\begingroup\makeatletter\ifx\SetFigFontNFSS\undefined%
\gdef\SetFigFontNFSS#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(1524,1524)(587,-695)
\end{picture}%


==> wl1.ins.tex <==
\begin{picture}(0,0)%
\includegraphics{wl1}%
\end{picture}%
\setlength{\unitlength}{3947sp}%
%
\begingroup\makeatletter\ifx\SetFigFontNFSS\undefined%
\gdef\SetFigFontNFSS#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(1524,1524)(587,-695)
\end{picture}%


==> wl2.ins.tex <==
\begin{picture}(0,0)%
\includegraphics{wl2}%
\end{picture}%
\setlength{\unitlength}{3947sp}%
%
\begingroup\makeatletter\ifx\SetFigFontNFSS\undefined%
\gdef\SetFigFontNFSS#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(1524,1524)(587,-695)
\end{picture}%


==> wlSum.ins.tex <==
\begin{picture}(0,0)%
\includegraphics{wlSum}%
\end{picture}%
\setlength{\unitlength}{3947sp}%
%
\begingroup\makeatletter\ifx\SetFigFontNFSS\undefined%
\gdef\SetFigFontNFSS#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(1524,1524)(587,-695)
\end{picture}%


==> zla.tex <==
%-*-EMaxima-*-
% см. ~/PA6OTA/MAXIMA/emaxima.tex
\input{header-landscape.tex}
\addtolength{\oddsidemargin}{.2cm}
\usepackage{emaxima}
% Чтобы следующие команды сработали, следует везде заменить:  \$ --> \var и убрать \mathrm
\newcommand{\varnt}{\tilde n} \newcommand{\varx}{x} \newcommand{\varxa}{x_a} \newcommand{\varxb}{x_b} \newcommand{\varm}{m} \newcommand{\vardel}{\delta}
\newcommand{\varDel}{\Delta} \newcommand{\varEFt}{\EF\tau}
% А ещё надо бы перейти от \pmatrix к \begin{pmatrix}...\end{pmatrix}
\begin{document}
\begin{maxima}
kill(mp,plusTOlist,xx,map2,fun,massiv,xi,pf,x,xa,xb,tau,Del,grinv,gainv,grp,grm,gap,gam,nt,m,EF,xiEF,EFt)$ declare([xi,t,ntildy],real)$
assume(tau>0,ntildy>0,m>0,EFt>0)$
plusTOlist(xx):=if atom(xx) then [xx] elseif op(xx)="+" then args(xx) elseif op(xx)="[" then xx else [xx]$
map2(fun,massiv):=map(lambda([xx],  map(fun, xx)), massiv)$
grinv:-xi+%i/(2*tau)$ gainv:conjugate(grinv)$ gr:1/grinv$ ga:1/gainv$
grp:1/(grinv+Del/2); grm:1/(grinv-Del/2)$ gap:1/(gainv+Del/2)$ gam:1/(gainv-Del/2)$
ntExpr:sqrt((1+del)*cos(phi)^2+(1-del)*sin(phi)^2);
\maximaoutput*
\m  {{1}\over{-\xi+{{i}\over{2\,\tau}}+{{\mathrm{\$Del}}\over{2}}}} \\
\m  \sqrt{\left(\cos \varphi\right)^2\,\left(\mathrm{\%del}+1\right)+\left(\sin \varphi\right)^2\,\left(1-\mathrm{\%del}\right)} \\
\end{maxima}
\begin{maxima}
res1:matrixmap(lambda([yy],block([resA,resB,resC],
resA:subst([xi=z/tau,EF=EFt/tau],subst([p=sqrt(2*m*(EF+EF*xiEF)),pf=sqrt(2*m*EF)],subst([px=p*cos(phi),py=p*sin(phi),Del=2*p*nt*x/(2*pf*tau)],yy))),
resB:map(factor,plusTOlist(subst([xiEF=z/EFt],ratdisrep(taylor(resA,xiEF,0,2))))),
resC:map(lambda([xx],factor(1/tau*integrate(xx,z,-inf,inf))),resB),
expand(1/(2*%pi)*integrate(subst([nt=ntExpr],apply("+",resC)),phi,0,2*%pi)))),
m/(2*%pi)*diag_matrix(px^2,py^2)/m^2*(grp*gap+grm*gam-2*gr*ga));
\maximaoutput*
\m  \begin{pmatrix}{{{\mathrm{\$x}^2\,\mathrm{\%del}}\over{4\,\mathrm{\$EFt}}}+{{\mathrm{\$x}^2}\over{2\,\mathrm{\$EFt}}}&0\cr 0&{{\mathrm{\$x}^2}\over{2\,\mathrm{\$EFt}}}-{{\mathrm{\$x}^2\,\mathrm{\%del}}\over{4\,\mathrm{\$EFt}}}\cr }\end{pmatrix} \\
\end{maxima}
\begin{maxima}
h[i,j]:=[(xa+xb)^2,(xa-xb)^2][i]/(2*pf*tau)^2*2*[px,py][i]*[px,py][j]/(Del*m)$
res2:matrixmap(lambda([yy],block([resA,resB,resC],
resA:subst([xi=z/tau,EF=EFt/tau],subst([p=sqrt(2*m*(EF+EF*xiEF)),pf=sqrt(2*m*EF)],subst([px=p*cos(phi),py=p*sin(phi),Del=2*p*nt*x/(2*pf*tau)],yy))),
resB:map(factor,plusTOlist(subst([xiEF=z/EFt],ratdisrep(taylor(resA,xiEF,0,2))))),
resC:map(lambda([xx],factor(1/tau*integrate(xx,z,-inf,inf))),resB),
expand(1/(2*%pi)*integrate(subst([nt=ntExpr],apply("+",resC)),phi,0,2*%pi)))),
m/(2*%pi)*genmatrix(h,2,2)*(grm*gam-grp*gap));
\maximaoutput*
\m  \begin{pmatrix}{-{{\mathrm{\$xb}^2}\over{4\,\mathrm{\$EFt}}}-{{\mathrm{\$xa}\,\mathrm{\$xb}}\over{2\,\mathrm{\$EFt}}}-{{\mathrm{\$xa}^2}\over{4\,\mathrm{\$EFt}}}&0\cr 0&-{{\mathrm{\$xb}^2}\over{4\,\mathrm{\$EFt}}}+{{\mathrm{\$xa}\,\mathrm{\$xb}}\over{2\,\mathrm{\$EFt}}}-{{\mathrm{\$xa}^2}\over{4\,\mathrm{\$EFt}}}\cr }\end{pmatrix} \\
\end{maxima}
\begin{maxima}
fiRes:subst([del=2*xa*xb/x^2],res1+res2);
fiRes[1,1]-fiRes[2,2];
\maximaoutput*
\m  \begin{pmatrix}{-{{\mathrm{\$xb}^2}\over{4\,\mathrm{\$EFt}}}-{{\mathrm{\$xa}^2}\over{4\,\mathrm{\$EFt}}}+{{\mathrm{\$x}^2}\over{2\,\mathrm{\$EFt}}}&0\cr 0&-{{\mathrm{\$xb}^2}\over{4\,\mathrm{\$EFt}}}-{{\mathrm{\$xa}^2}\over{4\,\mathrm{\$EFt}}}+{{\mathrm{\$x}^2}\over{2\,\mathrm{\$EFt}}}\cr }\end{pmatrix} \\
\m  0 \\
\end{maxima}
\end{document}

